Continuous Graph Flow

In this paper, we propose Continuous Graph Flow, a generative continuous flow based method that aims to model complex distributions of graph-structured data. Once learned, the model can be applied to an arbitrary graph, defining a probability density over the random variables represented by the graph. It is formulated as an ordinary differential equation system with shared and reusable functions that operate over the graphs. This leads to a new type of neural graph message passing scheme that performs continuous message passing over time. This class of models offers several advantages: a flexible representation that can generalize to variable data dimensions; ability to model dependencies in complex data distributions; reversible and memory-efficient; and exact and efficient computation of the likelihood of the data. We demonstrate the effectiveness of our model on a diverse set of generation tasks across different domains: graph generation, image puzzle generation, and layout generation from scene graphs. Our proposed model achieves significantly better performance compared to state-of-the-art models.

==> Continuous Graph Flow ICLR'20/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Continuous Graph Flow ICLR'20/sections/conclusion.tex <==
In this paper, we presented  \textit{continuous graph flow}, a generative model that generalizes the neural message passing in graphs to continuous time. We formulated the model as an neural ordinary differential equation system with shared and reusable functions that operate over the graph structure. We conducted evaluation for a diverse set of generation tasks across different domains: graph generation, image puzzle generation, and layout generation for scene graph. Experimental results showed that continuous graph flow achieves significant performance improvement over various of state-of-the-art  baselines. For future work, we will focus on generation tasks for large-scale graphs which is promising as our model is reversible and memory-efficient.
\newpage

==> Continuous Graph Flow ICLR'20/sections/experiments.tex <==
\vspace{-1mm}
To demonstrate the generality and effectiveness of our Continuous Graph Flow (CGF), we evaluate our model on three diverse tasks: (1) graph generation, (2) image puzzle generation, and (3) layout generation based on scene graphs. %As mentioned in Section~\ref{sec:cgf}, CGF can model continuous time dynamics of a set of graph variables including variables associated with edges, nodes or both. 
%First, we evaluate the effectiveness of CGF by modeling the variables associated with edges only and generate graph structure. Second, we generate variables associated with nodes given a graph structure for image puzzle generation and scene layout generation. 
Graph generation requires the model to learn complex distributions over the graph structure. Image puzzle generation requires the model to learn local and global correlations in the puzzle pieces. Layout generation has a diverse set of possible nodes and edges. These tasks have high complexity in the distributions of graph variables and diverse potential function types. Together these tasks pose a challenging evaluation for our proposed method.



\subsection{Graph Generation}
\vspace{-2mm}
\textbf{Datasets and Baselines. }We evaluate our model on graph generation on two benchmark datasets \textsc{ego-small} and \textsc{community-small}~\citep{you2018graphrnn} against four strong state-of-the-art baselines:  VAE-based method~\citep{simonovsky2018graphvae},  autoregressive graph generative model GraphRNN~\citep{you2018graphrnn} and DeepGMG~\citep{li2018learning}, and Graph normalizing flows ~\citep{liu2019gnf}. 

% mention that our model doesn't need to rely on an extra trained autoencoder

\textbf{Evaluation. } We conduct a quantitative evaluation of the generated graphs using Maximum Mean Discrepancy (MMD) measures proposed in \textsc{GraphRNN}~\citep{you2018graphrnn}.  The MMD evaluation in \textsc{GraphRNN} was performed using a test set of N ground truth graphs, computing their distribution over the nodes, and then searching for a set of N generated graphs from a larger set of samples generated from the model that best matches this distribution. As mentioned by~\cite{liu2019gnf}, this evaluation process would likely have high variance as the graphs are very small. Therefore, we also performed an evaluation by generating 1024 graphs for each model and computing the MMD distance between this generated set of graphs and the ground truth test set. Baseline results are from ~\cite{liu2019gnf}. Implementation details refer to Appendix A. 

\textbf{Results and Analysis. } Table~\ref{tb:graph_gen} shows the results in terms of MMD. Our CGF outperforms the baselines by a significant margin and also the concurrent work GNF. We believe our CGF outperforms GNF because it employs free-flow functions forms unlike GNF that has some contraints necessitated by the coupling layers. Fig.\ \ref{fig:graph_gen_2} visualizes the graphs generated by our model. Our model can capture the characteristics of datasets and generate diverse graphs that are not seen during the training. For additional visualizations and comparisons, refer to the Appendix A.

\begin{table}[h]
\caption{\textbf{Quantitative results on graph generation.} MMD measures between test set and generated graphs (lower is better). The second set shows \textsc{GraphRNN} evaluation with node distribution matching (averaged over 5 different models with 3 trials). The third set shows evaluation for the test set for all 1024 generated graphs (averaged over 5 models). (max$(|V|)$,max$(|E|)$) is also shown.}

\vspace{+1mm}
\centering
\begin{tabular}{l|ccc|ccc}
\hline
 \textbf{Method}& \multicolumn{3}{c}{\bf{\textsc{community-small}} (20,83)} \vline & \multicolumn{3}{c}{\bf{\textsc{ego-small}} (18,69)} \\
   & \textsc{Degree}  & \textsc{Clustering}  &  \textsc{Orbit}  & \textsc{Degree}  & \textsc{Clustering}  &  \textsc{Orbit}\\\hline 
\textsc{GraphVAE}   & 0.35 & 0.98 & 0.54 & 0.13 & 0.17 & 0.05  \\
\textsc{DeepGMG} & 0.22 & 0.95 & 0.4 & 0.04 & 0.10 & 0.02 \\
\hline
\textsc{GraphRNN} & 0.08& 0.12 &0.04 &0.09& 0.22& 0.003\\
\textsc{GNF} & 0.20 & 0.20 & 0.11 & 0.03 & 0.10 & 0.001\\
\textbf{CGF} & 0.10 & 0.30 & 0.08 & 0.02 & 0.11 & 0.001 \\
\hline
\textsc{GraphRNN (1024)} & 0.03& $\mathbf{0.01}$ &0.01 &0.04& 0.05& 0.06\\
\textsc{GNF (1024)} & 0.12 & 0.15 & 0.02 & 0.01 &0.03 &0.0008\\
\textbf{CGF (1024)} & %$\mathbf{0.02}$ & %$\mathbf{0.02}$ & %$\mathbf{0.001}$ & %$\mathbf{0.002}$ & %$\mathbf{0.007}$ & %$\mathbf{0.0002}$ 
$\mathbf{0.02}$ & 
0.02 & 
$\mathbf{0.001}$ &
$\mathbf{0.002}$ & 
$\mathbf{0.007}$ & 
$\mathbf{0.0002}$ \\
\hline
\end{tabular}
\label{tb:graph_gen}
\end{table}

\begin{figure}
    \centering
    \begin{tabular}{c|c}
        \includegraphics[width=0.47\textwidth,height=0.35\textwidth]{figs/results/graph_generation/caveman_samples.png} 
        &
      %\includegraphics[scale=0.2]{figs/results/graph_generation/citeseer_training.png} &
      \includegraphics[width=0.47\textwidth,height=0.35\textwidth]{figs/results/graph_generation/citeseer_samples.png} \\
      %\includegraphics[scale=0.2]{figs/results/graph_generation/caveman_training.png} &
    \textsc{community-small} &
      \textsc{ego-small} 
      \end{tabular}
    \vspace{-1mm}
    \caption{\textbf{Visualization of generated graphs from our model.} Our model can capture the characteristic of datasets and generate diverse graphs not appearing in the training set.}
    \label{fig:graph_gen_2}
    \vspace{-0.2in}
\end{figure}


\vspace{-1mm}
\subsection{Image puzzle generation}
\vspace{-1mm}
\label{subsec:puzzle_generation}
\textbf{Task description. } We design image puzzles for image datasets to test model's ability on fitting very complex node distributions in graphs. Given an image of size $W \times  W$, we design a puzzle by dividing the original image into non-overlapping unique patches. A puzzle patch is of size $w \times w$, in which $w$ represents the width of the puzzle. Each image is divided into $p=W/w$ puzzle patches both horizontally and vertically, and therefore we obtain $P=p\times p$ patches in total. Each patch corresponds to a node in the graph. To evaluate the performance of our model on dynamic graph sizes, instead of training the model with all nodes, we sample $\tilde{p}$ adjacent patches where $\tilde{p}$ is uniformly sampled from $\{1, \ldots ,P\}$ as input to the model during training and test. In our experiments, we use patch size $w =  16$, $p \in \{2,3,4\}$ and edge function for each direction (\textit{left}, \textit{right}, \textit{up}, \textit{down}) within a neighbourhood of a node. Additional details are in Appendix A.  

\textbf{Datasets and baselines.}  We design the image puzzle generation task for three datasets: MNIST~\citep{lecun1998gradient}, CIFAR10~\citep{krizhevsky2009learning}, and CelebA~\citep{liu2015deep}. CelebA dataset does not have a validation set, thus, we split the original dataset into a training set of 27,000 images and test set of 3,000 images as in~\citep{kingma2018glow}. %We perform training and testing using the training and validation set provided in the original dataset respectively. 
We compare our model with six state-of-the-art VAE based models: (1) StructuredVAE \citep{he2018variational}, (2) Graphite \citep{grover2018graphite}, (3) Variational message passing using structured inference networks (VMP-SIN) \citep{lin2018variational}, (4) BiLSTM + VAE: a bidirectional LSTM used to model the interaction between node latent variables (obtained after serializing the graph) in an autoregressive manner similar to \cite{gregor2015draw}, (5) Variational graph autoencoder (GAE)~\citep{kipf2016variational}, and (6) Neural relational inference (NRI)~\citep{kipf2018neural}: we adapt this to model data for single time instance and model interactions between the nodes.

\textbf{Results and analysis.} We report the negative log likelihood (NLL) in bits/dimension (lower is better). The results in Table~\ref{tb:puzzle_graph} indicate that CGF significantly outperforms the baselines.
In addition to the quantitative results, we also conduct sampling based evaluation and perform two types of generation experiments: (1) \textit{Unconditional Generation:} Given a puzzle size $p$, $p^2$ puzzle patches are generated using a vector $z$ sampled from Gaussian distribution (refer Fig.\ \ref{fig:conditional_celeb}(a)); and (2) \textit{Conditional Generation:} Given $p_1$ patches from an image puzzle having $p^2$ patches, we generate the remaining $(p^2 - p_1)$ patches of the puzzle using our model (see Fig.\ \ref{fig:conditional_celeb}(b)). We believe the task of conditional generation is easier than unconditional generation as there is more relevant information in the input during flow based transformations. For unconditional generation, samples from a base distribution (e.g. Gaussian) are transformed into learnt data distribution using the CGF model. For conditional generation, we map $\vec{x}_a \in \vec{X}_a$ where $\vec{X}_a \subset \vec{X}$ to the points in base distribution to obtain $\vec{z}_a$ and subsequently concatenate the samples from Gaussian distribution to $z_a$ to obtain $\vec{z}'$ that match the dimensions of desired graph and generate samples by transforming from $\vec{z}'$ to $\vec{x} \in \vec{X}$ using the trained graph flow. 
%Also, we cannot compare our model with existing flow based generative models because it is not possible to extend these models to flexible graph sizes.

%\greg{Why not train separate flow models for $p=2,3,4$?  Doesn't work for unseen sizes, but will for seen.}

%\zd{I though the point for this model was generalizability. Also for scene layout it's kind of hard to explicity train for just one single type of graph}

%\zd{Also I feel for this model it's more like instead of marginalizing over variables, we directly fit it. If we only know the joint distribution, we need to marginalize over variables, but if we can directly get the marginal distribution, maybe there's no point for marginalization.}

\begin{table}[!h]
\caption{\textbf{Quantitative results on image puzzle generation.} Comparison of our CGF model with standard VAE and state-of-the-art VAE based models in bits/dimension (lower is better). These results are for unconditional generation using multi-scale version of continuous graph flow.}
\centering
\vspace{+1mm}
\begin{tabular}{l|ccc|ccc|ccc}
\hline
 \textbf{Method}& \multicolumn{3}{c}{\textbf{MNIST}} \vline & \multicolumn{3}{c}{\textbf{CIFAR-10}} \vline & \multicolumn{3}{c}{\textbf{CelebA-HQ}} \\

   & 2x2  & 3x3 &   4x4& 2x2  & 3x3 &   4x4 &2x2  & 3x3 &   4x4\\\hline 
BiLSTM + VAE   & 4.97 &	4.77 & 4.42 & 6.02 & 5.20 & 4.53 & 5.72 & 5.66 & 5.48  \\
StructuredVAE~\citep{he2018variational}    & 4.89 & 4.65 & 3.82 & 6.03 & 5.02 & 4.70 & 5.66 & 5.43 & 5.27  \\
Graphite~\citep{grover2018graphite} & 4.90 & 4.64 & 4.02 & 6.06 & 5.09 & 4.61 & 5.71 & 5.50 & 5.32  \\
VMP-SIN~\citep{lin2018variational} & 5.13 & 4.92 & 4.44 & 6.00 & 4.96 & 4.34 & 5.70 & 5.43 & 5.27 \\
GAE~\citep{kipf2016variational}   & 4.91 &	4.89 & 4.17 & 5.83 & 4.95 & 4.21 & 5.71 & 5.63 & 5.28  \\
NRI~\citep{kipf2018neural} & 4.58 & 4.35 & 4.11 & 5.44 & 4.82 & 4.70 & 5.36 & 5.43 & 5.28  \\
\hline
CGF  &\textbf{1.24} &\textbf{1.21} & \textbf{1.20} & \textbf{2.42} &\textbf{2.31} & \textbf{2.00} &\textbf{3.44} &\textbf{3.17} &\textbf{3.16}\\ 
\hline
\end{tabular}
\label{tb:puzzle_graph}
\end{table}

\begin{figure}[!t]
\setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}{c @{\hskip 0.07in} @{\vrule width 1pt} @{\hskip 0.07in}c}
        \begin{tabular}{lllllll}
         \includegraphics[scale=0.65]{figs/results/unconditional/mnist1.jpg} &
         %\includegraphics[scale=0.65]{figs/results/unconditional/mnist2.jpg} &
         \includegraphics[scale=0.65]{figs/results/unconditional/mnist3.jpg} &
         \includegraphics[scale=0.65]{figs/results/unconditional/mnist5.jpg} &
         \includegraphics[scale=0.65]{figs/results/unconditional/mnist6.jpg} &
         \includegraphics[scale=0.65]{figs/results/unconditional/mnist7.jpg} &
         \includegraphics[scale=0.65]{figs/results/unconditional/mnist8.jpg} &
         \includegraphics[scale=0.65]{figs/results/unconditional/mnist4.jpg}
      \end{tabular}
      &
       \begin{tabular}{lllllll}
         \includegraphics[scale=1.3]{figs/results/conditional/mnist1.jpg} &
         \includegraphics[scale=1.3]{figs/results/conditional/mnist2.jpg} &
         \includegraphics[scale=1.3]{figs/results/conditional/mnist3.jpg} &
         \includegraphics[scale=1.3]{figs/results/conditional/mnist4.jpg} &
          \includegraphics[scale=1.3]{figs/results/conditional/mnist5.jpg} & 
         \includegraphics[scale=1.3]{figs/results/conditional/mnist6.jpg} 
         \includegraphics[scale=1.3]{figs/results/conditional/mnist7.jpg} &
         %\includegraphics[scale=1.4]{figs/results/conditional/mnist8.jpg}
      \end{tabular}
      \\
      \hline
      \\
        \begin{tabular}{llll}
         \includegraphics[scale=0.75]{figs/results/unconditional/celeba1.jpg} &
         \includegraphics[scale=0.75]{figs/results/unconditional/celeba2.jpg} &
         \includegraphics[scale=0.75]{figs/results/unconditional/celeba3.jpg} &
          \includegraphics[scale=0.75]{figs/results/unconditional/celeba4.jpg}
          \\
         \includegraphics[scale=0.75]{figs/results/unconditional/celeba5.jpg} &
         \includegraphics[scale=0.75]{figs/results/unconditional/celeba6.jpg} &
          \includegraphics[scale=0.75]{figs/results/unconditional/celeba7.jpg} &
         \includegraphics[scale=0.75]{figs/results/unconditional/celeba8.jpg}
         %\includegraphics[scale=0.75]{figs/results/unconditional/celeba9.jpg}
    \end{tabular}
         &
    \begin{tabular}{llll}
         \includegraphics[scale=1.5]{figs/results/conditional/celeba1.jpg} &
         \includegraphics[scale=1.5]{figs/results/conditional/celeba2.jpg} &
         \includegraphics[scale=1.5]{figs/results/conditional/celeba3.jpg} & 
          %\includegraphics[scale=1.5]{figs/results/conditional/celeba4.jpg} &
           \includegraphics[scale=1.5]{figs/results/conditional/celeba5.jpg}
         \\
         \includegraphics[scale=1.5]{figs/results/conditional/celeba6.jpg} &
          \includegraphics[scale=1.5]{figs/results/conditional/celeba7.jpg} &
         \includegraphics[scale=1.5]{figs/results/conditional/celeba8.jpg} &
         \includegraphics[scale=1.5]{figs/results/conditional/celeba9.jpg} 
      \end{tabular}
      \\
      (a) Unconditional Generation & (b) Conditional Generation
      \end{tabular}
    \vspace{-0.12in}
    \caption{\textbf{Qualitative results for image puzzle generation.} Samples generated using our model for 2x2 MNIST puzzles (above horizontal line) and 3x3 CelebA-HQ puzzles (below horizontal line) in (a) \textit{unconditional generation} and (b) \textit{conditional generation} settings. For setting (b), generated patches (highlighted in green boxes) are conditioned on the remaining patches (from ground truth).}
    \label{fig:conditional_celeb}
    \vspace{-0.22in}
\end{figure}
%\textbf{Generalization to unseen graph sizes. } To test the generalizability of our model to variable graph sizes (variable number of nodes), we design three different evaluation settings: (1) \textit{odd to even}: training with graphs having odd graph sizes and testing on graphs with even numbers of nodes, (2) \textit{less to more}: training on graphs with smaller sizes and testing on graphs with larger sizes, and (3) \textit{more to less}: training on graphs with larger sizes and testing on graphs with smaller. In the \textit{less to more} setting, we test the model's ability to use the factors learned from small graphs on more complicated ones, whereas the \textit{more to less} setting evaluates the model's ability to learn disentangled functions without explicitly seeing them during training. In our experiments, for the \textit{less to more} setting, we use sizes less than $G/2$ for training and more than $G/2$ for testing where G is the size of the full graph. Similarly, for the \textit{less to more} setting, we use sizes less than $G/2$ for training and more than $G/2$ for testing. Tab.\ \ref{tb:generalization} reports the NLL for these settings. The NLL of these models are close to the performance on the original experiments when trained with variable graph sizes indicating that our model is able to generalize to unseen graph sizes.
%\textbf{Baselines.} We compare the continuous graph flow with state-of-the-art likelihood based methods used for graphical modeling.
%\begin{itemize}
%    \item \textbf{VAE} \cite{kingma2013auto} Variational auto-encoder is used as a baseline which models each latent variable in the graph independently.
%    \item \textbf{GraphVAE} \cite{he2018variational} As there's no global structure to learn for flexible graphs, we use the fc variant of GraphVAE(which shows similar performance). The latent variables are modeled such that each variable is dependent on the parent variables.
%    \item \textbf{Graphite} \cite{gron2018graphite} Graphite is mainly used for graph edge modeling. In this paper, we adapt the model to modeling the graph nodes distribution by treating adjacency matrix as a latent variable too. The reparameterization is done by gumbel softmax.
%    \item \textbf{VMP-SIN} \cite{lin2018variational} incorporate the structure of the graphical model in the inference network of VAE. It also derives a variational message passing algorithm to perform efficient natural gradient inference while retaining the efficiency of the amortized inference.
%\end{itemize}
%\textbf{Number of message passing steps v.s. graph sizes} We here analyze the empirical relationships between number of adaptive message passing steps in graph flow and the size of graphs. Potentially, if a graph is complicated with larger number of nodes, the required message passing steps should be higher.
%\subsubsection{Generalization test}
%One core ability of graphical models is the ability to generalize to variable graph sizes. Here we test our model's generalization ability from three perspectives:
%\textbf{Odd to even}: We train our continuous graph flow model on graphs with odd graph sizes and test it's fitting ability on graphs with even number of nodes
%\textbf{Less to more}: We train our model on small graphs and test it on larger graphs. This is testing the model's ability on using the factors learned from small graphs to more complicated cases
%\textbf{More to less}: We train our model on large graphs and test it on small graphs. This tests the model to see whether it can learn disentangled functions/factors without explicitly using them as training.


%\textbf{Qualitative results. } We conduct two sets of generation experiments using continuous graph flow: (1) \textit{Unconditional Generation}: Given a puzzle size $p$, $p^2$ puzzle patches are generated using a vector $z$ sampled from Gaussian distribution (refer Figure~\ref{fig:conditional}(a)); and (2) \textit{Conditional Generation:} Given a $p_1$ patches from an image puzzle having $p^2$ patches, we generate the remaining $(p^2 - p_1)$ patches of the puzzle using our model (refer Figure~\ref{fig:conditional} (b)).

\vspace{-2mm}
\subsection{Layout generation from scene graphs}
\vspace{-2mm}
\textbf{Task description and evaluation metrics.} Layout generation from scene graphs is a crucial task in computer vision and bridges the gap between the symbolic graph-based scene description and the object layouts in the scene ~\citep{johnson2018image, bolayout, jyothi2019layoutvae}. Scene graphs represent scenes as directed graphs, where nodes are objects and edges give relationships between objects. Object layouts are described by the set of corresponding bounding box annotations~\citep{johnson2018image}. Our model uses scene graph as inputs (nodes correspond to objects and edges represent relations). An edge function is defined for each relationship type.  The output contains a set of object bounding boxes described by $\{[x_i, y_i, h_i, w_i]\}_{i=1}^n$, where $x_i, y_i$ are the top-left coordinates, and $w_i, h_i$ are the bounding box width and height respectively. We use negative log likelihood per node (lower is better) for evaluating models on scene layout generation.


%In general, this task is challenging because a single instance of a scene graph can potentially correspond to multiple instances of scene layouts. 

\textbf{Datasets and baselines. } Two large-scale challenging datasets are used to evaluate the proposed model: Visual Genome~\citep{krishna2017visual} and COCO-Stuff~\citep{caesar2018coco} datasets. Visual Genome contains 175 object and 45 relation types. The training, validation and test set contain 62565, 5506 and 5088 images respectively. %COCO-Stuff contains 80 things and 91 stuff categories.  %\textit{left of, right of, above, below, inside, and surrounding}. 
COCO-Stuff dataset contains 24972 train, 1024 validation, and 2048 test scene graphs.
We use the same baselines as in Sec.\ \ref{subsec:puzzle_generation}.
%We compare our model with standard VAE \cite{kingma2013auto} and three state-of-the-art VAE based models which focus on learning structured representations: (1) GraphVAE \cite{he2018variational}, (2) Graphite \cite{grover2018graphite}, and (3) Variational Message Passing using structured inference networks (VMP-SIN) \cite{lin2018variational}.

\begin{figure}
\centering
   \includegraphics[width=0.9\textwidth]{figs/vg_layouts_new.pdf}
   \vspace{-4mm}
   \caption{\textbf{Visualization for layout generation} on Visual Genome. Our CGF model can generate diverse layouts for the same scene graph. Upper row: layout samples with unconditional generation. Lower row: Layout generation conditioned on known layout. Best viewed in color. } %Please zoom in to see the category of each object.}
   \vspace{-0.22in}
   \label{fig:vg_layouts}
\end{figure}

\begin{table}[!h]
\caption{\textbf{Quantitative results for layout generation for scene graph} in negative log-likelihood. These results are for unconditional generation using CGF with generic message transformations.}
\centering
\vspace{+1mm}
\begin{tabular}{l|cc}
\hline 
\textbf{Method}     & \textbf{Visual Genome}   & \textbf{COCO-Stuff}    \\\hline 
% w/o clstm          &    &       & \\
BiLSTM + VAE    & -1.20 & -1.60 \\
StructuredVAE~\citep{he2018variational}     & -1.05  & -1.36 \\
Graphite~\citep{grover2018graphite} & -1.17 & -0.93 \\
VMP-SIN~\citep{lin2018variational} & -0.61 & -0.85 \\
GAE~\citep{kipf2016variational}    & -1.85 & -1.92 \\
NRI~\citep{kipf2018neural}  & -0.76 & -0.91 \\
\hline
CGF & \textbf{-4.24} & \textbf{-6.21}\\ 
%Ours - affine & & \\
\hline 
\end{tabular}
\vspace{-0.18in}
\label{tb:layout_generation}
\end{table}


\textbf{Results and analysis.} We show quantitative results in Table\ \ref{tb:layout_generation} against several state-of-the-art baselines. Our CGF model significantly outperforms these baselines in terms of negative log likelihood. Moreover, we show some qualitative results in 
Fig.\ \ref{fig:vg_layouts}. Our model can learn the correct relations defined in scene graphs for both conditional and unconditional generation, Furthermore, our model is capable to learn \textit{one-to-many} mappings and generate diverse of layouts for the same scene graph. 

\vspace{-2mm}
\subsection{Analysis: Generalization Test}
\vspace{-2mm}
To test the generalizability of our model to variable graph sizes, we design three different evaluation settings and test it on image puzzle task: (1) \textit{odd to even}: training with graphs having odd graph sizes and testing on graphs with even numbers of nodes, (2) \textit{less to more}: training on graphs with smaller sizes and testing on graphs with larger sizes, and (3) \textit{more to less}: training on graphs with larger sizes and testing on graphs with smaller. In the \textit{less to more} setting, we test the model's ability to use the functions learned from small graphs on more complicated ones, whereas the \textit{more to less} setting evaluates the model's ability to learn disentangled functions without explicitly seeing them during training. In our experiments, for the \textit{less to more} setting, we use sizes less than $G/2$ for training and more than $G/2$ for testing where G is the size of the full graph. Similarly, for the \textit{less to more} setting, we use sizes less than $G/2$ for training and more than $G/2$ for testing. Table\ \ref{tb:generalization} reports the NLL for these settings. The NLL of these models are close to the performance on the models trained on full dataset demonstrating that our model is able to generalize to unseen graph sizes.
\vspace{-0.2in}
\begin{table}[!h]
\caption{\textbf{Generalization test } in three different evaluation settings for image puzzle sizes 3x3 for three image datasets in bits/dimension.} %These results are for multiscale version of CGF.}
\centering
\vspace{+1mm}
\begin{tabular}{l|ccc}
\hline
 \textbf{Settings}&\textbf{MNIST}  & \textbf{CIFAR-10} & \textbf{CelebA-HQ} \\
 \hline
Odd to even &1.33  & 2.81 &3.31\\
Less to more &1.37  & 2.91 &3.66\\
More to less & 1.34 & 2.83 & 3.44\\
\hline
\end{tabular}
\label{tb:generalization}
\vspace{-0.18in}
\end{table}



==> Continuous Graph Flow ICLR'20/sections/intro_new.tex <==
Modeling and generating graph-structured data has important applications in various scientific fields such as building knowledge graphs~\citep{lin2015learning,bordes2011learning}, inventing new molecular structures~\citep{gilmer2017neural} and generating diverse images from scene graphs ~\citep{johnson2018image}. Being able to train expressive graph generative models is an integral part of AI research. 
%The desiderata of a powerful and expressive graph generative model include: (1) the ability to model diverse relations in the data, (2) the potential to model complex graph data distributions, and (3) flexibility to generate new instances of graphs with different dimensions. 

Significant research effort has been devoted in this direction. Traditional graph generative methods~\citep{erdHos1960evolution,leskovec2010kronecker,albert2002statistical,airoldi2008mixed} are based on rigid structural assumptions and lack the capability to learn from observed data. Modern deep learning frameworks within the variational autoencoder (VAE)~\citep{kingma2013auto} formalism offer promise of learning distributions from data. Specifially, for structured data, research efforts have focused on bestowing VAE based generative models with the ability to learn structured latent space models~\citep{lin2018variational,he2018variational,kipf2016variational}. Nevertheless, their capacity is still limited mainly because of the assumptions placed on the form of distributions. %Such assumptions are enforced by the approximations necessitated to handle intractability of exact likelihood computation.
Another class of graph generative models are based on autoregressive methods~\citep{you2018graphrnn,kipf2018neural}. These models construct graph nodes sequentially wherein each iteration involves generation of edges connecting a generated node in that iteration with the previously generated set of nodes. Such autoregressive models have been proven to be the most successful so far. However, due to the sequential nature of the generation process, the generation suffers from the inability to maintain long-term dependencies in larger graphs.
Therefore, existing methods for graph generation are yet to realize the full potential of their generative power, particularly, the ability to model complex distributions with the flexibility to address variable data dimensions.

Alternatively, for modeling the relational structure in data,
graph neural networks (GNNs) or message passing neural networks (MPNNs) ~\citep{scarselli2009graph, gilmer2017neural,duvenaud2015convolutional,li2017situation,kipf2016semi,santoro2017simple, zhang2018end} have been shown to be effective in learning generalizable representations over variable input data dimensions. These models operate on the underlying principle of iterative \textit{neural message passing} wherein the node representations are updated iteratively for a fixed number of steps. Hereafter, we use the term message passing to refer to this neural message passing in GNNs. We leverage this representational ability towards graph generation.
%graph neural networks (GNNs) or message passing neural networks (MPNNs) ~\citep{scarselli2009graph, gilmer2017neural,duvenaud2015convolutional,li2017situation,kipf2016semi,santoro2017simple, zhang2018end} are the most widely used frameworks. These models operate on the underlying principle of iterative \textit{message passing} wherein the node representations are updated iteratively for a fixed number of steps. %However, these models require saving the hidden states for all message passing steps leading to huge memory requirement. Recently proposed GRevNets alleviates the memory requirement but the message passing phase still comprises predetermined fixed number of message passing steps.

In this paper, we introduce a new class of models -- \textit{Continuous Graph Flow} (CGF): a graph generative model based on continuous normalizing flows~\citep{chen2018neural,grathwohl2018ffjord} that generalizes the message passing mechanism in GNNs to continuous time. Specifically, to model continuous time dynamics of the graph variables, we adopt a neural ordinary different equation (ODE) formulation. Our CGF model has both the flexibility to handle variable data dimensions (by using GNNs) and the ability to model arbitrarily complex data distributions due to free-form model architectures enabled by the neural ODE formulation. Inherently, the ODE formulation also imbues the model with following properties: reversibility and exact likelihood computation.

%- Since the model has no constrained forms, CGF has no model to obtain 

Concurrent work on Graph Normalizing Flows (GNF)~\citep{liu2019gnf} also proposes a reversible graph neural network using normalizing flows. However, their model requires a fixed number of transformations. In contrast, while our proposed CGF is also reversible and memory efficient, the underlying flow model relies on continuous message passing scheme. Moreover, the message passing in GNF involves partitioning of data dimensions into two halves and employs coupling layers to couple them back. This leads to several constraints on function forms and model architectures that have a significant impact on performance~\citep{kingma2018glow}. In contrast, our CGF model has unconstrained (free-form) Jacobians, enabling it to learn more expressive transformations.

We demonstrate the effectiveness of our CGF-based models on three diverse tasks: graph generation, image puzzle generation, and layout generation based on scene graphs. Experimental results show that our proposed model achieves significantly better performance than state-of-the-art models.
\begin{figure}
   \centering
   \includegraphics[width=0.9\textwidth]{figs/model_figure_new1.pdf}
   %\vspace*{-0.15in}
   \vspace{-0.15in}
   \caption{Illustration of evolution of message passing mechanisms from discrete updates (a) to our proposed continuous updates (b). Continuous Graph Flow leverages normalizing flows to transform simple distributions (e.g. Gaussian) at $t_0$ to the target distributions at $t_1$. The distribution of only one graph node is shown here for visualization, but, all the node distributions transform over time. }
   \vspace{-0.15in}
   \label{fig:pullfig}
\end{figure}

==> Continuous Graph Flow ICLR'20/sections/model_1.tex <==
\section{Preliminaries}
\textbf{Graph neural networks. } %Deep relational networks such as graph neural networks (GNNs) facilitate learning highly nonlinear interactions between nodes with high dimensions by using complex neural networks functions. Specifically, 
Relational networks such as Graph Neural Networks (GNNs) facilitate learning of non-linear interactions using neural networks. 
In every layer $\ell \in \mathbb{N}$ of a GNN, the embedding $\vec{h}_i^{(\ell)}$ corresponding to a graph node accumulates information from its neighbors of the previous layer recursively as described below.
%\greg{Isn't $l\in \mathbb{N}$, discrete for GNNs?}
%\greg{Use $\ell$ instead of $l$, it's easier to read.}
%\greg{$\vec{x_i}$ should be used above}
\begin{equation}
    \vec{h}_i^{(\ell)} = g\bigg(\bigg\{f_{ij}(\vec{h}_i^{(\ell-1)}, \vec{x}_i^{(\ell-1)}, \vec{x}_j ^{(\ell-1)}) | j \in \mathcal{S}(i) \bigg\}\bigg),
\end{equation}
where the function $g$ is an aggregator function, $\mathcal{S}(i)$ is the set of neighbour nodes of node $i$, and $f_{ij}$ is the message function from node $j$ to node $i$, ${\vec{x}_i}^{(\ell-1)}$ and ${\vec{x}_j}^{(\ell-1)}$ represent the node features corresponding to node $i$ and $j$ at layer $(\ell-1)$ respectively. Our model uses a restricted form of GNNs where embeddings of the graph nodes are updated in-place ($\vec{x}_i \leftarrow \vec{h}_i$), thus, we denote graph node as $\vec{x}$ and ignore $\vec{h}$ hereafter. These in-place updates allow using $\vec{x}_i$ in the flow-based models while maintaining the same dimensionality across subsequent transformations.

%Our model uses the form of GNN where embeddings of the graph nodes are kept the same across iterations. This allows using $\vec{x}_i$ in the flow-based models (below) while maintaining the same dimensionality across iterations.


%Our model uses a restricted form of GNN where embeddings of the graph nodes are updated in-place ($\vec{x}_i \leftarrow \vec{h}_i$), thus, we use $\vec{x}$ for the graph node representation and ignore $\vec{h}$ hereafter. This in-place update allows using $\vec{x}_i$ in the flow-based models (below) while maintaining the same dimensionality across iterations.

%Graph neural networks are often used as deep feature extractor and are followed by a mean field distribution. It doesn't support flexible inference or complex distribution modeling. %\mn{do we upfront provide definitions of flexible inference?otherwise, flexible inference sounds very vague}
%\greg{Confusion here between inputs and random variables, observed and latent random variables.}

\textbf{Normalizing flows and change of variables. } 
Flow-based models enable construction of complex distributions from simple distributions (e.g. Gaussian) through a sequence of invertible mappings~\citep{rezende2015variational}. For instance, a random variable $\vec{z}$ is transformed from an initial state density $\vec{z}_0$ to the final state $\vec{z}_K$  using a chain of $K$ invertible functions $f_k$ described as:
\begin{equation}
    \vec{z}_K = f_K \circ \ldots f_2 \circ f_1 (\vec{z}_0).
\end{equation}

The computation of log-likelihood of a random variable uses change of variables rule formulated as:
\begin{equation}
    \log p_K(\vec{z}_K) = \log p_0(\vec{z}_0) - \sum_{k=1}^{K}\log \bigg|\det\frac{\partial f_k (\vec{z}_{k-1})}{\partial \vec{z}_{k}}\bigg|,
    \label{eq:cov}
\end{equation}
where $\partial f_k (\vec{z}_{k-1})/\partial \vec{z}_{k} $ is the Jacobian of $f_k$ for $k \in \{1, 2, ...,K\}$. 

\textbf{Continuous normalizing flows. }Continuous normalizing flows (CNFs)~\citep{chen2018neural, grathwohl2018ffjord} model the continuous-time dynamics by pushing the limit on number of transformations. 
Given a random variable $\vec{z}$, the following ordinary differential equation (ODE) defines the change in the state of the variable.
\begin{equation}
    \frac{\partial{\vec{z}}}{\partial{t}} = f(z(t),t)
\end{equation}
\cite{chen2018neural} extended the change of variables rule described in Eq.~\ref{eq:cov} to continuous version. The dynamics of the log-likelihood of a random variable is then defined as the following ODE.
\begin{equation}
    \frac{\partial{p(\vec{z}(t)}}{\partial{t}} = Tr\bigg(\frac{\partial f}{\partial \vec{z}(t)}\bigg)
    \label{eq:trace}
\end{equation}
Following the above equation, the log likelihood of the variable $z$ at time $t_1$ starting from time $t_0$ is
\begin{equation}
    \log p(\vec{z}(t_1)) = \log p(\vec{z}(t_0)) - \int_{t_0}^{t_1}Tr\bigg(\frac{\partial f(\vec{z})}{\partial \vec{z}(t)}\bigg),
\end{equation}
where the trace computation is more computationally efficient than computation of the Jacobian in Equation (4). Building on CNFs, we present continuous graph flow which effectively models continuous time dynamics over graph-structured data.

\section{Continuous graph flow}
\label{sec:cgf}
Given a set of random variables $\vec{X}$ containing $n$ related variables, the goal is to learn the joint distribution $p(\vec{X})$ of the set of variables $\vec{X}$. Each element of set $\vec{X}$ is $\vec{x}_i \in \mathbb{R}^{m}$ where $i = 1,2\ldots,n$ and $m$ represents the number of dimensions of the variable.  %These set of related variables can be any set of variables, for instance, nodes, edges or both of a graph.
%We model the interactions between the graph variables as a set of message functions $\{f_a\}, a \in \mathcal{A}$ which takes a subset of graph variables as input and produces an aggregated message from other variables to the target variable. 
For continuous time dynamics of the set of variables $\vec{X}$, we formulate an ordinary differential equation system as follows:
\begin{equation}
  \begin{bmatrix}
    \vec{\dot x}_{1}(t)\\
    \vec{\dot x}_{2}(t)\\
    \vdots\\
    \vec{\dot x}_{n}(t)
  \end{bmatrix}
=
  \begin{bmatrix}
    f^1(\vec{X}(t))\\
    f^2(\vec{X}(t))\\
    \vdots\\
    f^n(\vec{X}(t))
  \end{bmatrix},
\end{equation}

where $\vec{\dot x_i} =  d \vec{x}_i/dt$ and $\vec{X}(t)$ is the set of variables at time $t$. The random variable $\vec{x}_i$ at time $t_0$ follows a base distribution that can have simple forms, \textit{e.g.} Gaussian distributions. The function $f^i$ implicitly defines the interaction among the variables.
%\begin{equation}
%\frac{d \vec{x_i}(t)}{dt} = f_a(\{\vec{x}_a(t)\},t,\theta)
%   \log p(\vec{X}(t_1)) = \log p(\vec{X}(t_0)) + \int_{t_0}^{t_1}F(\vec{X}(t), t, \theta)dt
%\end{equation}
Following this formulation, the transformation of the individual graph variable is defined as
\begin{equation}
      \vec{x}_i(t_1) = \vec{x}_i(t_0) + \int_{t_0}^{t_1}f^i(\vec{X}(t)) dt ,
      \label{eqn:full_ode}
      \end{equation}
This provides transformation of the value of the variable $\vec{x_i}$ from time $t_0$ to time $t_1$. %The joint distribution of variables $p(\vec{X})= p(\vec{x_1},\ldots ,\vec{x_{n}})$ is the data distribution to be learned. %The base distributions $\vec{x_i}(t_0) \sim q(\vec{x_i}(t_0))$ can have simple forms such as Gaussian distributions.

%\zd{check whether fast adaptation still makes sense}


\subsection{Continuous message passing} 
\label{sec:cmp}
The form in Eq.~\ref{eqn:full_ode} represents a generic multi-variate update where interaction functions are defined over all the variables in the set $\vec{X}$. However, the functions do not take into account the relational structure between the graph variables.% and the form of update functions $f(\cdot)$ does not naturally permit generalization to new random variables.

To address this, we define a neural message passing process that operates over a graph by defining the update functions over variables according to the graph structure. This process begins from time $t_0$ where each variable $\vec{x}_i(t_0)$ only contain local information. At time $t$, these variables are updated based on the information gathered from other neighboring variables. For such updates, the function $f^i$ in Eq.~\ref{eqn:full_ode} is defined as: 
\begin{equation}
    f^i(\vec{X}(t)) = g(\{\hat{f}_{ij}(\vec{x}_{i}(t),\vec{x}_{j}(t)) | j \in \mathcal{S}(i)\}),
\end{equation}
where $\hat{f}_{ij}(\cdot)$ is a reusable message function and used for passing information between variables $\vec{x_i}$ and $\vec{x_j}$, $\mathcal{S}(i)$ is the set of neighboring variables that interacts with variable $\vec{x_i}$, and $g(\cdot)$ is a function that aggregates the information passed to a variable. The above formulation describes the case of pairwise message functions, though this can be generalized to higher-order interactions. %\mn{still not sure if the last sentence makes sense - revisit the function}

We formulate it as a continuous process which eliminates the requirement of having a predetermined number of steps of message passing. By further pushing the message passing process to update at infinitesimally smaller steps and continuing the updates for an arbitrarily large number of steps, the update associated with each variable can be represented using shared and reusable functions as the following ordinary differential equation (ODE) system.
\begin{equation}
  \begin{bmatrix}
    \vec{\dot x}_{1}(t)\\
    \vec{\dot x}_{2}(t)\\
    \vdots\\
    \vec{\dot x}_{n}(t)
  \end{bmatrix}
=
  \begin{bmatrix}
    g(\{\hat{f}_{1j}(\vec{x}_{1}(t),\vec{x}_{j}(t)) | j \in \mathcal{S}(1)\})\\
    g(\{\hat{f}_{2j}(\vec{x}_{2}(t),\vec{x}_{j}(t)) | j \in \mathcal{S}(2)\})\\
    \vdots\\
    g(\{\hat{f}_{nj}(\vec{x}_{n}(t),\vec{x}_{j}(t)) | j \in \mathcal{S}(n)\})\\
  \end{bmatrix},
\end{equation}
%\begin{equation}
%\begin{aligned}
%\frac{d\vec{x}_i(t)}{dt} &= g\bigg(\bigg\{f_a(\{\vec{x}_{a}(t)\})\bigg\}\bigg),  a\in \mathcal{A}, i \in \{1,2,...,N\} \\
%\end{aligned}
%\label{eq: system}
%\end{equation}
where $\vec{\dot x_i} =  d \vec{x}_i/dt$. %We implement this as a fixed library of functions, the selection from which $a(\cdot,\cdot)$ depends on the type of node to allow for generalization to new graph structures. 
Performing message passing to derive final states is equivalent to solving an initial value problem for an ODE system. Following the ODE formulation, the final states of variables can be computed as follows. This formulation can be solved with an ODE solver.
\begin{equation}
    \vec{x}_i(t_1) = \vec{x}_i(t_0) + \int_{t_0}^{t_1}g\bigg(\bigg\{\hat{f}_{ij}(\vec{x}_{i}(t),\vec{x}_{j}(t)) | j \in \mathcal{S}(i)\bigg\}\bigg),  i \in \{1,\ldots,n\}.
\end{equation}

%\mn{Why write this below? Instead say it can be done with uniform step-size or adaptive step-size as shown in neuralODE. memory efficient doesn't fit in the definition section and reads like an overselling statement}
%\zd{This part should go to related works or introduction while acknowledging the contribution of NeuralODE. Temporarily put it here.} %Nonetheless, we can potentially benefit from FFJORD framework \cite{grathwohl2018ffjord} that can perform message passing with adaptive stepsize for computing the above integral, \textit{i.e.}, the ODE solver can adjust the number of steps needed according to the states of the system. 

%Also, the continuous message passing block has high memory efficiency.
\subsection{Continuous message passing for density transformation}
\vspace{-1mm}
%In this work, we introduce a powerful graph flow that can fit the complex graphical distributions though using continuous message passing as implicit density transformation. 
Continuous graph flow leverages the continuous message passing mechanism (described in Sec.\ \ref{sec:cmp}) and formulates the message passing as implicit density transformations of the variables (illustrated in Figure~\ref{fig:pullfig}). Given a set of variables $\vec{X}$ with dependencies among them, the goal is to learn a model that captures the distribution from which the data were sampled. 
Assume the joint distribution $p(\vec{X})$ at time $t_0$ has a simple form such as independent Gaussian distribution for each variable $\vec{x}_i(t_0)$. The continuous message passing process allows the transformation of the set of variables from $\vec{X}(t_0)$ to $\vec{X}(t_1)$. Moreover, this process also converts the distributions over variables from simple base distributions to complex data distributions. Building on the \textit{independent variable} continuous time dynamics described in Eq.~\ref{eq:trace}, we define the dynamics corresponding to related \textit{graph variables} as:
\begin{equation}
    \frac{\partial \log p(\vec{X}(t))}{\partial t} = -Tr\bigg(\cfrac{\partial F}{\partial \vec{X}(t)}\bigg),
\end{equation}
where %the set of variables $\vec{X}$ is a concatenation of all variables $\vec{x}_i$ in the graph (varies depending on the size of the input graph) and 
$F$ represents a set of reusable functions incorporating aggregated messages. %Following Eq. 5, the change in log-likelihood along with the sequential changes of variables can be reduced to the trace computation of Jacobian matrix $\partial F/\partial \vec{X}(t)$~\citep{chen2018neural}.
Therefore, the joint distribution of set of variables $\vec{X}$ can be described as:
\begin{equation}
    \log p(\vec{X}(t_1)) = \log p(\vec{X}(t_0)) - \int_{t_0}^{t_1}Tr\bigg(\frac{\partial F}{\partial \vec{X}(t)}\bigg).
    \label{eq:density}
\end{equation}


Here we use two types of density transformations for message passing: (1) \textit{generic message transformations} -- transformations with generic update functions where trace in Eq.~\ref{eq:density} can be approximated instead of computing by brute force method, and (2) \textit{multi-scale message transformations} -- transformations with generic update functions at multiple scales of information.

%\textbf{Affine Message Transformation} We define a simple closed form of the update function as follows.

%\begin{equation}
%    \frac{d\vec{x}_i(t)}{dt} = f_u(\vec{x}_i(t)) + \vec{s}(\{\vec{x}_j(t)\})\cdot %\vec{x}_i(t) + \vec{b}(\{\vec{x}_j(t)\})
%\end{equation}

%where the function $f_u$ is the self transformation function of variable $\vec{x}_i(t)$ and can be implemented by functions used in single-variable flow methods (\textit{e.g.} affine coupling, 1x1 convolution) and the functions $\vec{b}$ and $\vec{s}$ are computed using the neighbourhood variables $\{\vec{x}_j\}$ serving as relational information between the variable and its neighbours.

%Note that in conventional flow-based methods, this update method is computationally expensive due to the to calculation of the determinant of Jacobian matrix of the transformation function. In contrast, this transformation only requires the trace of logarithm of the Jacobian matrix that can be easily computed as $\sum_{d} \vec{s}_d + Tr(\partial f_u / \partial \vec{x}_i)$ where $d$ denotes the dimension of $\vec{s}$.

\textbf{Generic message transformations. } The trace of Jacobian matrix in Eq.~\ref{eq:density} is modeled using a generic neural network function. The likelihood is defined as:
\begin{equation}
    \log p(\vec{X}(t_1)) = \log p(\vec{X}(t_0)) - \mathbb{E}_{p(\vec{\epsilon})}\int_{t_0}^{t_1}\bigg[\vec{\epsilon}^T\frac{\partial F}{\partial \vec{X}(t)}\vec{\epsilon}dt\bigg],
\end{equation}

where $F$ denotes a neural network for message functions, and $\vec{\epsilon}$ is a noise vector and usually can be sampled from standard Gaussian or Rademacher distributions.

%\textbf{Multi-head continuous gate dynamics}

%\mn{explain below}

\textbf{Multi-scale message transformations. } As a generalization of generic message transformations, we design a model with multi-scale message passing to encode different levels of information in the variables. Similar to ~\cite{dinh2016density}, we construct our multi-scale CGF model by stacking several blocks wherein each flow block performs message passing based on generic message transformations. After passing the input through a block, we factor out a portion of the output and feed it as input to the subsequent block. The likelihood is defined as: 
\begin{equation}
    \log p(\vec{X}(t_{b})) = \log p(\vec{X}(t_{b-1})) - \mathbb{E}_{p(\vec{\epsilon})}\int_{t_{b-1}}^{t_{b}}\bigg[\vec{\epsilon}^T\frac{\partial F}{\partial \vec{X}(t_{b-1})}\vec{\epsilon}dt\bigg],
\end{equation}
where $b = 1,2, \ldots,(B-1)$ with $B$ as the total number of blocks in the design of the multi-scale architecture. Assume at time $t_b$ ($t_0 < t_b < t_1$), $\vec{X} (t_b)$ is factored out into two. We use one of these (denoted as $\tilde{\vec{X}} (t_b)$) as the input to the $(b+1)^{\text{th}}$ block. Let $\tilde{\vec{X}}(t_b)$ be the input to the next block, the density transformation is formulated as:
\begin{equation}
    \log p(\tilde{\vec{X}}(t_{b+1})) = \log p(\tilde{\vec{X}}(t_{b})) - \mathbb{E}_{p(\vec{\epsilon})}\int_{t_{b}}^{t_{b+1}}\bigg[\vec{\epsilon}^T\frac{\partial F}{\partial \tilde{\vec{X}}(t_{b})}\vec{\epsilon}dt\bigg].
\end{equation}

%\zd{Will add adjoint part soon}
%\subsection{Backpropagation with adjoint method}

%\subsection{Flexible graph inference}
%With the ability of modeling joint distributions over graph variables, we can easily (\zd{can we say something about the complexity of this inference -- to be checked}) perform the conditional distribution inference and marginal distribution inference over graphs. Here we present two ways of inference/evaluation once we are able to learn a powerful flow-based graph model.

%Modeling of joint distributions over graph variables enables conditional inference and marginal distribution evaluation over certain subsets of variables in the graphical model.

%\textbf{Conditional inference.} Existing likelihood-based methods on graphical models approximate the data distributions based on the observed data samples and offer limited inference capabilities due to the approximations learned during training. In contrast, flow-based models provide the ability to compute exact likelihood of the data distribution. 
%Therefore, given the learned graph flow model on the set of variables $\vec{X} = \{\vec{x}_i\}_{i=1}^n$, it is straightforward to compute the distribution of any subset of variables $\vec{X}_a \subset \vec{X}$ conditioned over other variables $\vec{X}_b \subset \vec{X}$ by $p(\vec{X}_a|\vec{X}_b) = p(\vec{X}_a, \vec{X}_b)/p(\vec{X}_b)$. In particular, we map $\vec{x}_a$ to the latent space to obtain $\vec{z}_a$, we concatenate the samples from Gaussian distribution to $z_a$ to obtain $\vec{z}'$ that match the dimensions of graph and perform a backward transformation from $\vec{z}'$ to $\vec{x} \in \vec{X}$.

%\mn{@ \textbf{greg}: any better way to write this or choose not to include this? we don't explicitly say this anywhere in experiments but it is done implicitly in generalization test}\\
%\greg{I don't quite follow the exact marginal computation.  Sampling is fine.  But for exact marginal, how does this work?  How do we integrate over all latent variables in the flowed complex distribution?  If there isn't a clear answer, omit this section and just state in the experiments that evaluations is via a sampling process.}
%\textbf{Marginal distribution evaluation and sampling.} Given a set of variables $\vec{X} = \{\vec{x}_i\}$, sampling from a marginal distribution over any subset of variables $\vec{X}_a \subset \vec{X}$ can simply be performed on the initial variables $\vec{X}_a(t_1) \sim p(\vec{X}_a(t_0))$ then the samples are transformed to the final data distribution. The evaluation of probability can be done using a backward transformation from time $t_1$ to $t_0$.

%\subsection{Fast adaptation based graph inference}
%In many applications, the name of node variables in a graph is not known and requires separate fitting for different graph instances. We present a need to simple extended version of our graph flow model for handling this situation. We propose a \textit{model agnostic meta learning based continuous graph flow} to fastly adapt to any new coming graph. This fast adaptation starts from latent variables which fastly move from unit Gaussian to some new Gaussian distributions, then propagate to the node variable space. Function parameters can either remain fixed or also be adapted by per graph, depending on whether functions are shared across graph instances.
%\mn{ this is very confusing for even me as an author}
%\zd{Will need to think more about this}


==> Continuous Graph Flow ICLR'20/sections/rw.tex <==
%Our work builds on the prior research work in the fields of : (1) probabilistic graphical models, (2) generative modeling, (3) learning structured representations, and (4) learning graph representations. In this section, we discuss the existing related work relevant to the flow based generative models.

\mn{Make it discussion and related work combined}

\textbf{Probabilistic graphical models. } Probabilistic graphical models (PGMs) serve as a statistical framework for modeling dependencies among random variables and building multivariate statistical models \cite{wainwright2008graphical}. Traditional modeling algorithms include belief propagation networks \cite{yedidia2001generalized, ping2017belief,murphy1999loopy}, Markov Random Fields \cite{rue2005gaussian,boykov1998markov,ishikawa2003exact}, Conditional Random Fields (CRFs) \cite{lafferty2001conditional,zheng2015conditional,quattoni2007hidden} and Restricted Boltzmann Machines (RBMs) \cite{sutskever2009recurrent,hinton2012practical}. Neural networks have also been explored for inference in PGMs to model the inference steps as feedforward or recurrent networks \cite{li2014mean,dai2016discriminative}. Based on the similarities in the message passing mechanism of graph neural networks (GNNs) and iterative updates for dependencies between variables in PGMs \cite{gilmer2017neural}, we use GNN based architectures to represent graphical models in our work.

\textbf{Generative modeling.} Recent generative modeling techniques such as autoregressive methods \cite{oord2016pixel,van2016wavenet}, variational autoencoders (VAEs) \cite{kingma2013auto, lin2018variational,he2018variational,grover2018graphite,kipf2016variational,kipf2018neural} and generative adversarial networks (GANs) \cite{goodfellow2014generative} have demonstrated considerable success in modeling complex data distributions. These models focus on learning a joint probability distribution over variables in the data. However, none of these models allow exact computation of likelihood of the data. More recently, flow-based generative models \cite{rezende2015variational,kingma2018glow,dinh2014nice,dinh2016density} have been designed allowing the computation of exact likelihood of the data. %However, these models often have several constraints on their architectures to reduce the computational complexity. %Another class of models that propose a continuous time version of normalizing flows which replaces the warping function with an integral of continuous-time dynamics are capable of relaxing the constraints on the model architecture \cite{chen2018neural,grathwohl2018ffjord}. Nonetheless, the effectiveness of these models have only been demonstrated for dynamics involving single variable and do not model dependencies among different variables. In contrast, we apply the flow based methods to multi-variate dynamics to procure distributions that incorporate statistical dependencies in complex graphical models. 
Continuous time of normalizing flows \cite{chen2018neural,grathwohl2018ffjord} allow flow-based models to have completely unrestricted architectures, but have been shown to be effective for modeling dynamics for a single variable(with coherent meaning). In this work, we use continuous normalizing flows to model the multivariate dynamics to procure data distributions that incorporate statistical dependencies in complex graphical models.

\textbf{Learning structured representations. } Recently, there has been a surge of interest in modeling efforts that focus on improving generative models with the ability to learn structured latent space by unifying PGMs and VAEs~ \cite{lin2018variational, he2018variational,johnson2016composing, simonovsky2018graphvae}. However, these models still have limited capacity mainly because they are based on approximate computation of likelihood of data.   

\textbf{Learning graph representations. }% Graphs are ubiquitous data structure and have been extensively employed in various domains, including social networks \cite{tang2015line, hamilton2017inductive}, knowledge graphs \cite{nickel2016review, velivckovic2017graph, hamaguchi2017knowledge}, visual reasoning \cite{yao2018exploring, johnson2018image}, neural machine translation \cite{marcheggiani2018exploiting, beck2018graph}, chemical prediction \cite{gilmer2017neural}, and protein-protein interactions \cite{velivckovic2017graph, fout2017protein}. 
%Learning representations on graphs that encode structural information about the graph has proved extremely useful for a wide variety of tasks, including social networks \cite{tang2015line, hamilton2017inductive}, knowledge graphs \cite{nickel2016review, velivckovic2017graph, hamaguchi2017knowledge}, visual reasoning \cite{yao2018exploring, johnson2018image}, neural machine translation \cite{marcheggiani2018exploiting, beck2018graph}, chemical prediction \cite{gilmer2017neural}, and protein-protein interactions \cite{velivckovic2017graph, fout2017protein}. 
%These graph representation learning approaches optimize the mapping of embedding nodes or (sub)graphs into a low-dimensional vector space so that geometric relationships in the embedding space represent the structure of the original graph \cite{hamilton2017representation}. 
Random walk approaches \cite{perozzi2014deepwalk, grover2016node2vec}, factorization-based approaches \cite{belkin2002laplacian, cao2015grarep} and GNN based approaches \cite{scarselli2009graph, velivckovic2017graph, kipf2016semi} are three main approaches for representation learning on graphs. Our work is closely related with GNNs, in which nodes repeatedly accumulate information from their neighbors in a recursive manner. %Several variants of GNNs have been proposed based on heuristics and empirical validation that achieve state-of-the-art performance on tasks such as node classification, link prediction, and graph classification \cite{duvenaud2015convolutional,li2017situation,kipf2016semi,santoro2017simple,santoro2018measuring, zhang2018end}. Nonetheless, these variants are limited in their capacity to fit the data distributions due to the assumptions on the model architecture such as predetermined number of nodes. 
However, as opposed to the conventional discrete time updates, our model employs continuous normalizing flow based techniques to build flexible graph representations.  






